$\Omega$-symmetric measures and related singular integrals

Let $\mathbb{S} \subset \mathbb{C}$ be the circle in the plane, and let $\Omega: \mathbb{S} \to \mathbb{S}$ be an odd bi-Lipschitz map with constant $1+\delta_\Omega$, where $\delta_\Omega>0$ is small. Assume also that $\Omega$ is twice continuously differentiable. Motivated by a question raised by Mattila and Preiss in [MP95], we prove the following: if a Radon measure $\mu$ has positive lower density and finte upper density almost everywhere, and the limit $$ \lim_{\epsilon \downarrow 0} \int_{\mathbb{C} \setminus B(x,\epsilon)} \frac{\Omega\left((x-y)/|x-y|\right)}{|x-y|} \, d\mu(y) $$ exists $\mu$-almost everywhere, then $\mu$ is $1$-rectifiable. To achieve this, we prove first that if an Ahlfors-David 1-regular measure $\mu$ is symmetric with respect to $\Omega$, that is, if $$ \int_{B(x,r)} |x-y|\Omega\left(\frac{x-y}{|x-y|}\right) \, d\mu(y) = 0 \mbox{ for all } x \in \mbox{spt}(\mu) \mbox{ and } r>0, $$ then $\mu$ is flat, or, in other words, there exists a constant $c>0$ and a line $L$ so that $\mu= c \mathcal{H}^{1}|_{L}$.

==> 04_SYM_smallbeta.tex <==
\section{Case when $\beta$'s are small} \

Let $A$ be as in \eqref{eq:SYM:r} and let $N \sim \log(A)$; fix $Q \in \mucubes$ and let $x_0$ and $x_1$ be the balanced points in $Q$ guaranteed by Lemma \ref{lemma:SYM_balancedcubes}. We will assume throughout this section that 
\begin{align} \label{eq:SYM_betasmall}
    \sum_{k=0}^N \beta_2(B(x_0, 2^k \ell(Q)) \leq \tau, 
\end{align}
where $\tau>0$ is a small constant which will be fixed later.


It will be convenient for us to define the $C_{\Omega, \phi}$ quantity in terms of a smooth cut off of the annulus $A(0, \frac{1}{2}, 2)$: let $\chi_\frac{1}{2}$ be a smooth radial function supported on $B(0,1)$ and so that $B\ps{0, \frac{1}{2}} \leq \chi_{\frac{1}{2}} \leq \chara_{B(0,1)}$; let $\chi_1$ be the same smooth radial function rescaled so that $\chara_{B(0,1)}\leq \chi_1\leq \chara_{B(0,2)}$.  We set
\begin{align} \label{eq:SYM_smoothcut}
    \phi:= \chi_1 - \chi_{\frac{1}{2}}.
\end{align}
Then we see that, for $r>0$, $\phi\ps{\av{ \frac{x-\cdot}{r}}^2}$ is supported on $A\ps{x, \frac{r}{2}, 2r}$. 

Recall Lemma \ref{lemma:SYM_borelequiv} and Remark \ref{remark:SYM_borelequiv}: $C_{\Omega, \phi}(x,r) = 0$ if and only if $C_{\Omega}(x,r)=0$; throughout this section we will work with the quantity $C_{\Omega, \phi}$ with $\phi$ as in \eqref{eq:SYM_smoothcut}.


\subsection{Lower bounds on the linear component $\mathbf{T}$} \

We denote by $\Pi_L$ the standard orthogonal projection onto the line $L$. 
\begin{lemma} \label{lemma:SYM_Tlowerbound}
Fix a $\mu$-cube $Q$ and let $x_0, x_1$ be balanced points of $Q$ and $L$ be the respective balanced plane. Let $T$ be defined as in \eqref{eq:GK_T} with $\phi$ as in \eqref{eq:SYM_smoothcut}. For any $z \in 3 Q$, set $e_z:= \frac{z-\Pi_L(z)}{|z- \Pi_L(z)|}$. If \eqref{eq:SYM_betasmall} holds, we have  
\begin{align}
    - \langle T(e_z), \nu \rangle \gtrsim \frac{1}{r},
\end{align}
where $\nu$ is the unit normal to $K(L)$. 
\end{lemma}

Without loss of generality, we can prove this lemma with $x_0 = 0$; let $z \in 3Q$ and set $\bar z := \Pi_L(z)$.
Let us look at the quantity
\begin{align*}
    \langle T(e_z), \nu \rangle & = \langle A_2(e_z), \nu \rangle + \langle B_{1,2,1}(e_z), \nu \rangle. 
\end{align*}
Recall the definition of $T$ in \eqref{eq:GK_T}. We will first take care of the term containing $A_2$ and later the one containing $B_{1,2,1}$.

\subsubsection{Control of $A_2$.}
Recall that the term $A_2$ is given by
\begin{align*}
\frac{1}{r} \int \frac{DK(-y) \cdot x }{r}\phi\left(\left|\frac{K(y)}{r}\right|^2\right) \, d \mu(y).
\end{align*}
\begin{remark} \label{remark:SYM_rm1}
Let us mention that, writing (for fixed $y$) $e_z^{\parallel (y)}$ (resp. $e_z^{\bot (y)}$) for the parallel (resp. orthogonal) component of $e_z$ with respect to $y$, 
$
    \langle y/|y|, e_z \rangle \Omega(y) = \left( \langle y/|y|, e_z^{\parallel (y)}\rangle \right) \Omega(y)$, since clearly $\left< y, e_z^{\perp(y)}\right>=0$; 
Similarly, $|y| D\Omega(y) e_z = |y|D \Omega(y) e_z^{\bot (y)}$. 
\end{remark}

\begin{sublemma} \label{sublemma:SYM_lower_bounde_A2}
Let $\delta_0 = \cos(\pi/2-\delta_1)$, with $\delta_1 \leq \pi/6$. Then
\begin{align}
    - \left< A_2(e_z), \nu \right> \gtrsim  \frac{\delta_0^2}{r}.
\end{align}
\end{sublemma}

\begin{proof}
By the product rule, we have 
\begin{align}
    -\langle A_2(e_z), \nu \rangle  & = \frac{1}{r} \int \frac{\langle \langle D(|y|), e_z\rangle \, \Omega(y), \nu \rangle }{r}\phi\left(\left|\frac{y}{r}\right|^2\right) \, d \mu(y)\\
    & \enskip  + \frac{1}{r} \int \frac{\langle |y| D\Omega(y)
\cdot e_z, \nu \rangle }{r}\phi\left(\left|\frac{y}{r}\right|^2\right) \, d \mu(y).  \label{eq:GK_lineartermA2b}
\end{align}
The first term in the last equation above equals to 
\begin{align}
    \frac{1}{r} \int \frac{\langle y/|y|, e_z\rangle \times |y|^{-1} \left< K(y), \nu\right> }{r}\phi\left(\left|\frac{y}{r}\right|^2\right) \, d \mu(y). \label{eq:GK_lineartermA2}
\end{align}
Suppose first that 
\begin{align} \label{eq:SYM_dotprod1}
  |y| \geq \left<y, e_z \right> \geq |y| \delta_0  
\end{align}
| with 
\begin{align} \label{eq:SYM_delta0}
    \delta_0= \delta_0(\delta_1) := \cos\ps{\frac{\pi}{2} - \delta_1 };
\end{align}
here $\delta_1$ is a positive, small constant to be fixed later. Since $\Omega(e_x) \perp \nu$, we have 
\begin{align}
    \cos(|\Omega(y)- \arg(\nu)|) =\sin(|\Omega(y)- \Omega(e_x)|). 
\end{align} 
Let us denote by $\alpha$ the angle $|\arg(y)- \arg(e_x)|$; as $\Omega: [0, 2\pi] \to [0, 2\pi]$ is bi-Lipschitz with constant $1+ \delta_\Omega$,
\begin{align} \label{eq:SYM_sinOmega}
    \sin(|\Omega(y)- \Omega(e_x)|) \geq \sin\left(\frac{1}{1+ \delta_\Omega}\alpha\right).
\end{align}
If we Taylor expand the right hand side of \eqref{eq:SYM_sinOmega} at $\alpha$, we have
\begin{align}
    \sin((1+\delta_\Omega)^{-1} \alpha) = \sin(\alpha) + \cos(\xi_{\alpha, \delta_\Omega})\frac{(-\alpha \delta_\Omega)}{1+ \delta_\Omega}, 
\end{align}
where $\xi_{\alpha, \delta_\Omega} \in [(1+\delta_\Omega)^{-1}\alpha, \alpha]$.
Note that, by \eqref{eq:SYM_dotprod1}, $\pi/2 \geq \alpha \geq \delta_1$: from this we have  that  $0 \leq \cos(\xi_{\alpha, \delta_\Omega}) \leq \cos(\delta_1)$. Hence we see that 
\begin{align} \label{eq:SYM_dotprods2}
    \sin(\alpha) - \cos(\delta_1) \frac{\alpha \delta_\Omega}{1+ \delta_\Omega}.
\end{align} 
We want something that looks like 
\begin{align}\label{eq:SYM_dotprod3}
    \eqref{eq:SYM_dotprods2} \geq \frac{1}{2} \sin(\alpha);
\end{align} 
if this held, we could conclude that if $\left<y, e_z \right> \geq |y| \delta_0$, then also $\left< K(y), \nu \right> \geq |y|\delta_0/2$.
One can check that  \eqref{eq:SYM_dotprod3} holds whenever
\begin{align} \label{eq:SYM_cond_on_Lip}
    \delta_\Omega \leq \frac{\cos(\delta_1)}{\pi - \cos(\delta_1)}.
\end{align}
Consider now $|y|\left< D\Omega(y) \cdot e_z, \nu\right>$; by Remark \ref{remark:SYM_rm1}, $D\Omega(y) \cdot e_z = D\Omega(y) \cdot e_z^{\perp (y)}$. Now, $e_z^{\perp (y)} = \left< y^\perp |y|^{-1}, e_z \right> \frac{y^\perp}{|y|}$. But notice that the operator $y \mapsto y^\perp$ is just a rotation, thus an isometry. Hence $\left< y^\perp, e_z\right> = \left<y, e_x\right>$. This observation let us re-write $|y|\left< D\Omega(y) \cdot e_z, \nu\right>$ as 
\begin{align}
    |y| \left<y, e_x\right>\, |y|^{-2}\left<D\Omega(y)\cdot y^\perp, \nu \right>  & = |y|^{-2} \left<y, e_x\right> \left< K(y)^\perp, \nu \right> \\
    & = |y|^{-2} \left<y, e_x \right> \left< K(y), \Omega(e_x)\right>,
\end{align}
recalling that $\nu^\perp= \Omega(e_x)$ by definition. 
Now, assume first that $|y| \geq \left< y, e_x \right> \geq |y|\delta_0$, with $\delta_0$ as in \eqref{eq:SYM_delta0}.
    Then we have that
    \begin{align*}
        \cos\ps{|\Omega(y) - \Omega(e_x)|} \geq \cos \ps{(1+\delta_\Omega)|\arg(y)-\arg(e_x)|}
    \end{align*}
    Again, set  $\alpha: =|\theta(y)-\theta(e_x)|$. If we Taylor expand the term on the right hand side, we see that
    \begin{align*}
    \cos \ps{(1+\delta_\Omega)\alpha } = \cos\ps{\alpha}- \sin(\xi_{\alpha, \delta_\Omega}) \delta_\Omega\alpha,
    \end{align*}
    where $\xi_{\alpha, \delta_\Omega} \in [\alpha, \alpha(1+ \delta_\Omega)]$. Thus
    \begin{align*}
        \cos\ps{(1+\delta_\Omega)\alpha} \geq \delta_0 - \delta_\Omega \alpha.
    \end{align*}
    Clearly, by our assumption on $\left< y, e_x\right>$,  $\alpha$ must be less that $ \frac{\pi}{2} - \delta_1$, and therefore we can estimate 
    \begin{align} \label{eq:SYM_posiA}
        \cos\ps{(1+\delta_\Omega) \alpha} \geq \cos(\pi/2- \delta_1) - \delta_\Omega (\pi/2- \delta_1).
    \end{align}
    We would like to have $\cos(\pi/2-\delta_1) - \delta_\Omega(\pi/2-\delta_1) \geq \frac{\cos(\pi/2-\delta_1)}{2}$; this will be the case if 
    \begin{align} \label{eq:SYM_smallLip}
        \delta_\Omega \leq \frac{\cos\ps{\frac{\pi}{2} - \delta_1}}{2\ps{\frac{\pi}{2} - \delta_1}}= \frac{\sin(\delta_1)}{2\ps{\frac{\pi}{2} - \delta_1}}
    \end{align}

Note that if $|y| \geq \left< y, -e_x \right> \geq \delta_0$ (resp. $|y| \geq \left< y, -e_z \right> \geq \delta_0 |y|$), then 
\begin{align} \label{eq:SYM_symmetry}
& \left< K(y), \Omega(-e_x) \right>= - \left< K(y), \Omega(e_x) \right> \geq \frac{\delta_0}{2} \\
& \mbox{resp.  } - \left< K(y), \nu \right> \geq \frac{\delta_0}{2}.
\end{align}

Thus, we may write
\begin{align}
    & \int\left( \left< K(-y), e_{\Omega(x)}\right> \left< y, e_x \right> + \left< K(-y), \nu \right> \left<y, e_z\right> \right) \frac{\phi\ps{\av{\frac{y}{r}}^2}}{| y|^2} \, d\mu(y) \label{eq:SYM_int0}\\
    & = \int_{\{|\left< y, e_x \right>| \geq \delta_0 |y| \, \mathrm{ and } \, |\left< y, e_z \right>| \geq \delta_0 |y|\}} \label{eq:SYM_int1}\\
    & + \int_{\{|\left< y, e_x\right>| \leq \delta_0 |y|\, \mathrm{but } \, |\left<y, e_z\right>| \geq \delta_0 |y| \}} \label{eq:SYM_int2}\\
    & + \int_{\{|\left< y, e_z\right>| \leq \delta_0 |y|\, \mathrm{but } \, |\left<y, e_x\right>| \geq \delta_0 |y| \}}. \label{eq:SYM_int3}
\end{align}
Indeed, notice that we cannot possibly have that both $|\left<y, e_x\right>| \leq \delta_0 |y|$ and $|\left<y, e_z\right>| \leq \delta_0 |y|$.
The integral in \eqref{eq:SYM_int1} can be immediately bounded below by
\begin{align}
    & \frac{1}{r^2}\int_{\{|\left< y, e_x \right>| \geq \delta_0 |y| \, \mathrm{ and } \, |\left< y, e_z \right>| \geq \delta_0 |y|\}} \delta_0^2 |y|^2 \frac{\phi\ps{\av{\frac{y}{r}}^2}}{|y|^2}\, d\mu(y) \\
    & \geq \frac{\delta_0^2}{r^2} \mu(\{|\left< y, e_x \right>| \geq \delta_0 |y| \, \mathrm{ and } \, |\left< y, e_z \right>| \geq \delta_0 |y|\} \cap A(0, r, 2r)). \label{eq:SYM_int4}
\end{align}
As for the integral in \eqref{eq:SYM_int2}, we proceed as follows: by choosing $\delta_1>0$ appropriately, we can make sure that if 
\begin{align} \label{eq:SYM_111}
    |\left<y, e_x \right>| \leq \delta_0 |y|= \cos(\pi/2 - \delta_1)|y|,
\end{align}
then $|\left<K(y), \Omega(e_x)\right>| \leq 2 \delta_0 |y|$; thus for any $y$ satisfying \eqref{eq:SYM_111}, we have that
\begin{align}
    \left<y, e_x\right> \left<K(y), K(e_x)\right> \geq - 3\delta_0^2 |y|^2.
\end{align}
On the other hand, still for those $y$'s such that \eqref{eq:SYM_111} holds, we have that
\begin{align}
    \cos(|\theta(y) - \theta(e_x)|)  \geq \sin\ps{\frac{\pi}{2}- \delta_1}. 
\end{align}
Hence we may write
\begin{align}
    & \int_{\{|\left< y, e_x\right>| \leq \delta_0 |y|\, \mathrm{but } \, |\left<y, e_z\right>| \geq \delta_0 |y| \}} \ps{ \left<y, e_x\right> \left<K(y), K(e_x)\right> + \left<y, e_z\right>\left<K(y), \nu\right> } \frac{\phi\ps{\av{\frac{y}{r}}^2}}{| y|^2} \, d\mu(y) \\
    & \gtrsim \int_{\{|\left< y, e_x\right>| \leq \delta_0 |y|\, \mathrm{but } \, |\left<y, e_z\right>| \geq \delta_0 |y| \}} |y|^2\ps{ - \cos^2\ps{\frac{\pi}{2}-\delta_1}  + \sin^2 \ps{\frac{\pi}{2} - \delta_1} } \frac{\phi\ps{\av{\frac{y}{r}}^2}}{| y|^2} \, d\mu(y)\\
    & = \int_{\{|\left< y, e_x\right>| \leq \delta_0 |y|\, \mathrm{but } \, |\left<y, e_z\right>| \geq \delta_0 |y| \}} \ps{1 - 2 \cos^2\ps{\frac{\pi}{2} - \delta_1}} \, \phi\ps{\av{\frac{y}{r}}^2} \, d\mu(y). \label{eq:SYM_121}
\end{align}
If we choose $\delta_1 \leq \frac{\pi}{6}$ (which determines $\delta_\Omega$), we obtain that 
$1 - 2 \sin(\delta_1) \geq \frac{1}{2}$, and therefore 
\begin{align} \label{eq:SYM_A230}
    \eqref{eq:SYM_121} \geq \frac{1}{2} \mu \ps{\{|\left< y, e_x\right>| \leq \delta_0 |y|\, \mathrm{but } \, |\left<y, e_z\right>| \geq \delta_0 |y| \} \cap A(0, r, 2r)}.
\end{align}
We can estimate the integral in \eqref{eq:SYM_int3} in the same way; the three estimates together and the lower regularity of $\mu$ give the sublemma.
\end{proof}
\begin{remark}
Note that the constant $\delta_1>0$ decides what are the convenient hypothesis on $\delta_\Omega$: we will have to take
\begin{align}
    \delta_\Omega \leq \frac{3}{4\pi}, 
\end{align}
so that both \eqref{eq:SYM_cond_on_Lip} and \eqref{eq:SYM_smallLip} are satisfied. 
\end{remark}

\subsubsection{Control of $B_{1,2,1}$}
Recall that $B_{1,2,1}(x)$ is given by 
\begin{align*}
    \frac{1}{r} \int \frac{K(-y)}{r}\phi'\left(\left|\frac{y}{r}\right|^2\right) \left[ \left< \frac{K(-y)}{r}, \frac{DK(-y) \cdot x }{r} \right>\right] \, d \mu(y)
\end{align*}
\begin{sublemma}\label{lemma:SYM_bound_on_B121}
\begin{align} \label{eq:SYM_bound_on_B121}
    - \int_{B(0,r)} \dist(y, L_Q)^2 r^{-4}\, d\mu(y) \leq \left<B_{1,2,1}(e_z), \nu\right> \leq \int_{B(0,r)} \dist(y, L_Q)^2 r^{-4} \, d\mu(y).
\end{align}
\end{sublemma}
\begin{proof}
As before, we split the integral into the radial derivative and the spherical one. That is, 
\begin{align}
    B_{1,2,1}(x) & = \frac{1}{r} \int \frac{K(y)}{r}\phi'\left(\left|\frac{y}{r}\right|^2\right) \left[ \langle \frac{K(y)}{r}, \frac{\langle y/|y|, e_z \rangle \Omega(y)}{r} \rangle\right] \, d \mu(y) \\
    & + \frac{1}{r} \int \frac{K(y)}{r}\phi'\left(\left|\frac{y}{r}\right|^2\right) \left[ \langle \frac{K(y)}{r}, \frac{|y| D \Omega(-y) e_z}{r} \rangle\right] \, d \mu(y)\\
    & =: I(x) + II(x).
\end{align}
Let us first compute $\langle I(e_z), \nu \rangle$. We have
\begin{align*}
\langle I(e_z), \nu \rangle & = \frac{1}{r} \int \frac{\langle K(y), \nu\rangle}{r} \phi' \left(\left|\frac{y}{r}\right|^2\right) 
\left[ \langle \frac{K(y)}{r}, \frac{\langle y/|y|, e_z \rangle \Omega(y)}{r} \rangle\right] \, d \mu(y).
\end{align*}
The second inner product in the integral can be re-written as
\begin{align*}
    & \langle y/|y|, e_z \rangle \langle r^{-1}K(y) , r^{-1} \Omega(y) \rangle \\
    & = \frac{\langle y, e_z \rangle }{r^2} 
\end{align*}
Hence we obtain
\begin{align} \label{eq:GKB121}
    \langle I(e_z), \nu \rangle = \frac{1}{r^4} \int \left<y, e_z\right> \left< K(y), \nu \right> \phi'\, d\mu(y).
\end{align}
Using Lemma \ref{lemma:SYM_dotprods}, we see that
\begin{align}
    - \int_{B(0,r)} \dist(y, L_Q)^2 r^{-4}\, d\mu(y) \leq \eqref{eq:GKB121} \leq \int_{B(0,r)} \dist(y, L_Q)^2 r^{-4} \, d\mu(y).
\end{align}

Let us now look to compute $\langle II(e_z), \nu \rangle$. We see that $D\Omega(y) \cdot e_z \in T_{\Omega(y)}\mathbb{S}^1$. Thus
\begin{align*}
\langle K(y) , |y|D\Omega(y) \cdot e_z \rangle = 0,
\end{align*}
and so $\langle II(e_z), \nu \rangle =0$. 
\end{proof}

\begin{corollary} \label{corollary:SYM_lowerbound}
\begin{align*}
    & \langle A_2(e_z) + B_{1,2,1}(e_z) , \nu \rangle \\
    & \gtrsim   \frac{\delta_0^2}{r}-\frac{2}{r^2} \int_{B(0,r)} \left( \frac{\dist(y, L_{Q})}{r}\right)^2  \, d \mu(y).
\end{align*}
\end{corollary}
\begin{proof}
This follows at once from Lemma \ref{sublemma:SYM_lower_bounde_A2} and \ref{lemma:SYM_bound_on_B121}.
\end{proof}

We divert for a moment from the main argument, to delve a little more in the choice of the balanced cubes $x_0$ and $x_1$. The following definition will be used later on. 
For a point $y \in \spt(\mu)$, set
\begin{align}
    \beta(y, Q) := \ps{\int_{A \ell(Q)}^{2A \ell(Q)} \beta_{2,\mu}(x,r)^2 \, \dr}^{\frac{1}{2}}.
\end{align}

\begin{lemma} \label{lemma:GK_goodpoints}
There exists a constant $c^*>0$ such that the following holds. Let $Q \in \mucubes$ and let $P(Q)$ be the line minimising $\beta_{\mu,2}(Q)$;  we can choose $x_0$ and $x_1$ as in Lemma \ref{lemma:SYM_balancedcubes} so that first,
\begin{align}
    \dist(x_j, P(Q)) \leq c^* \beta_{\mu, 2}(Q) \ell(Q), \, \, j=0,1,
\end{align}
and second,
\begin{align}
    \beta(x_j, Q)^2 \leq c^* \fint_Q \beta(y, Q)^2 \, d\mu(y), \,\, j=0,1.
\end{align}
\end{lemma}
\begin{proof}
Let $y_0, y_1 \in Q$ be the balanced points guaranteed by Lemma \ref{lemma:SYM_balancedcubes} and, for a constant $0< \eta<1$ to be fixed later, let $B_j$ denote $B(y_j, \eta \ell(Q)) \cap Q$. For two constants $c, c'>0$, we set
\begin{align*}
    & F_j(a):= \left\{ y \in B_j |\dist(y, P(Q)) \leq c\, \beta_{\mu, 2}(Q)\right\},\\
    & G_j(b) := \left\{ y \in B_j | \, \beta(y, Q)^2 \leq c'\,  \fint_Q \beta(y, Q)^2 \, d\mu(y) \right\}.
\end{align*}
By Chebyshev inequality and Cauchy - Schwarz, we have, for $j=0,1$, 
\begin{align} \label{eq:SYM_cheby_Fj}
    \mu(B_j \setminus F_j) & = \mu\ps{\left\{y \in B_j\, |\, \ell(Q)^{-1} \dist(y,P(Q)) > c \, \beta_{\mu,2}(Q) \right\}} \nonumber \\
    & \leq \frac{1}{c \, \beta_{\mu,2}(Q)} \, \int_{\{\ell(Q)^{-1} \dist(y, P(Q)) > c\, \beta_{\mu,2}(Q)\}} \frac{\dist(y, P(Q))}{\ell(Q)} \, d\mu(y) \nonumber\\
    & \leq  \frac{1}{c \, \beta_{\mu,2}(Q)} \mu(B_Q)^{\frac{1}{2}} \ps{\int_{B_Q} \ps{\frac{\dist(y, P(Q))}{\ell(Q)}}^2 \, d\mu(y) }^{\frac{1}{2}} \nonumber \\
    & \lesssim \frac{\mu(B_Q)}{c}.
\end{align}
Note that by Ahlfors regularity, we have that $\mu(B_Q)\lesssim \frac{1}{\eta} \mu(B_j)$.
Similarly, we have
\begin{align} \label{eq:SYM_cheby_Gj}
    \mu(B_j \setminus G_j) & \leq \frac{1}{c' \fint_Q \beta(y, Q)^2 d\mu} \int_Q \beta(y, Q)^2 \, d\mu = \frac{\mu(Q)}{c'} \lesssim \frac{\mu(B_j)}{c' \eta}.
\end{align}
We want to show that, for $c, c'$ large enough, we have that $F_j \cap G_j \neq \emptyset$; we argue by contradiction and we assume that for all $c, c'$ the intersection is empty. By \eqref{eq:SYM_cheby_Fj} and \eqref{eq:SYM_cheby_Gj}, we have
\begin{align}
    \frac{\eta r}{c_0} \leq \mu(B_j)  \leq \mu(B_j \setminus F_j) + \mu(B_j \setminus G_j) \leq \mu(B_j)\ps{\frac{1}{c \eta} + \frac{1}{c' \eta} } \leq c_0 r \ps{\frac{1}{c}+\frac{1}{c'}}.
\end{align}
This is clearly a contradiction. Thus for $c,c'$ large enough (depending only on $\eta$ and $c_0$), we see that $F_j \cap G_j \neq \emptyset$. Taking $c^*= c^*(\eta, c_0) := \max\{c,c'\}$ we end the proof of the lemma. 
\end{proof}

\begin{proof}[Proof of Lemma \ref{lemma:SYM_Tlowerbound}]
Now, we see that
\begin{align} \label{eq:GK_distl0}
\dist(y, L_Q) \leq \dist(y, L_{B(0, r)}) + \dist_H\left( L_{B(0, r)} \cap B(0, r), L_Q \cap B(0, r)\right), 
\end{align}
and, using Lemma \ref{lemma:GK_goodpoints}, that
\begin{align} \label{eq:GK_distl0b}
\dist_H\left( L_{B(0, r)} \cap B(0, r), L_Q \cap B(0, r)\right) \lesssim r \, \sum_{k=0}^N \beta_{\mu, 2} (0, 2^k \ell(Q)),
\end{align}
with $N \sim \log_2(A)$.
Recalling that $\mu$ is ADR, we have that
\begin{align*}
& r^{-1} \, \int_{B(0, r)} \left( \frac{\dist(y, L_Q)}{r}\right)^2 \, d\mu(y) \\
& \lesssim r^{-1} \int_{B(0, t)} \left( \frac{\dist(y, L_{B(0, r)})}{r}\right)^2 \, d\mu(y)\\
& \enskip \enskip + r^{-1} \, \int_{B(0, r)} \left( \sum_{k=0}^N \beta_{\mu, 2}(0, 2^k \ell(Q))\right)^2 \, d\mu(y) \\
& \lesssim \beta_{\mu, 2}(0, 2^k \ell(Q))^2 + \frac{\mu(B(0, r))}{r} \left(\sum_{k=0}^N \beta_{\mu, 2}(0, 2^k \ell(Q))\right)^2 \\
& \lesssim \left(\sum_{k=0}^N \beta_{\mu, 2} (0, 2^k \ell(Q))\right)^2.
\end{align*}
Hence 
\begin{align*}
    \frac{1}{ r^{1+1}} \int_{B(0, r)} \frac{\dist(y,L_0)^2}{r^2} \, d\mu(y)  \lesssim \frac{1}{ r} \, \left(\sum_{k=0}^N \beta_{\mu,2}(0, 2^k\ell(Q))\right)^2 \lesssim \frac{\tau^2}{r}.
\end{align*}
Using Corollary \ref{corollary:SYM_lowerbound}, we finally obtain
\begin{align} \label{eq:SYM_Tlowerbound}
    - \langle T(e_z) , \nu\rangle \geq C \left( \frac{\delta_0^2c_0}{r} - \frac{\tau^2}{r} \right) \geq \frac{C(\delta_0, \tau)}{2r}.
\end{align}
An appropriate choice of $\tau$ and $\delta_0$ gives the lemma.
\end{proof}

\subsection{Upper bound on the (nonlinear) error term $\mathbf{E}$} 

Keep the same notation as above. In this subsection we will prove an upper bound for the error term $E$ in terms of distance to the balanced plane $L_Q$. 
\begin{lemma} \label{lemma:GK_errorx}
Let $x_0, x\in Q$ be balanced points so that $x \in Q \setminus \frac{1}{2}Q $. Let $\nu$ be the unit vector normal to $K(L_{Q})$. Then 
\begin{align}
    |\left< E(x), \nu \right>| \lesssim \frac{|x|^2}{r^4} \int_{B(x_0,r)} \dist(y, L_{Q}) \, d\mu(y).
\end{align}
\end{lemma}

We will prove the lemma in the following several paragraphs; each paragraph corresponds to a piece of $E$.

\begin{remark}
We will assume below that $x_0=0$, witout loss of generality.
\end{remark}

\subsubsection{Estimates on $A_3$} \label{subsection:GK_A3}
Recall that 
\begin{align*}
    A_3(x) = \frac{1}{r} \int \frac{x^T D^2(K(\xi_{x, 0}-y)) x}{r} \, \phi\left(\left| \frac{y}{r}\right|^2\right) \, d\mu(y).
\end{align*}
In order to estimate this term, we need to understand the integrand
    \begin{align*}
        x^T D^2 K(\xi_{x,0} -y) x = \left(x^T D^2 K_1(\xi_{x,0} -y) x\,, \, x^T D^2 K_2(\xi_{x,0} -y) x \right)^T.
    \end{align*}
For $i=1,2$, and writing $\xi_{x,0} -y= \xi_{x,0,y}=:\xi$, we apply the product rule:
    \begin{align}
        D^2 K_i(\xi) 
        & = (D^2|\xi|) \Omega_i (\xi) +  \left(\left(D|\xi|\right)^T\, D \Omega_i (\xi)+ D(|\xi|) \left(D \Omega_i(\xi)\right)^T \right)^T  + |\xi| D^2\Omega_i(\xi)\\
        & =: I_i + II_i + III_i.
    \end{align}
We write $I=(I_1,I_2)^T \in \C$, and similarly for $II$ and $III$.     
\subsubsection{Bounds for $I$}    
    Let us look at $|\langle (I_1, I_2)^T, \nu\rangle|$. We see that 
    \begin{align*}
        &\langle [ x^T D^2(|\xi|) \Omega_1(\xi) x , x^T D^2( |\xi|) \Omega_2(\xi) x ], \nu \rangle\\
        & =\left( \frac{1}{|\xi|} \langle K(\xi), \nu\rangle\right) x^T D^2( |\xi| )x \, . 
    \end{align*}
    Now, on one hand, using Lemma \ref{lemma:SYM_dotprods}, $\left|\frac{1}{|\xi|} \langle K(\xi), \nu\rangle\right| \sim \frac{\dist(\xi, L_{Q})}{|\xi|}$. On the other hand, 
    \begin{align*}
        |x^T D^2(|\xi|) x| \sim |x|^2 \frac{1}{|\xi|}.
    \end{align*}
    Hence, 
    \begin{align*}
        |\langle (I_1, I_2)^T, \nu\rangle| \lesssim \frac{\dist(\xi, L_Q) |x|^2}{|\xi|^2}.
    \end{align*}
    Therefore, 
    \begin{align*}
        & \frac{1}{r} \int \left| \frac{ \langle [ x^T D^2|\xi| \Omega_1 (\xi) x , x^T D^2 |\xi| \Omega_2(\xi) x ], \nu \rangle}{r} \right| \phi\ps{\av{\frac{y}{r}}^2} \, d\mu(y) \\
        & \lesssim \frac{|x|^2}{r^4} \int_{B(0,r)} \dist(y, L_{Q}) \, d\mu(y).
    \end{align*}
    \subsubsection{Bounds for $II$} We now look at $\langle (II_1, II_2)^T , \nu\rangle$. 
    To do so, we consider first the term $\left(D|\xi|\right)^T D \Omega_i (\xi)$. The other one can be dealt with in the same fashion. 
    First, notice that, for $i =1,2$, 
    \begin{align*}
        x^T (D|\xi|)^T D\Omega_i(\xi) x = \langle x, D|\xi| \rangle \langle D \Omega_i(\xi) , x \rangle.
    \end{align*}
    Thus we have that
    \begin{align} \label{eq:SYM_ErrorB_1}
        \left< \left(x^T (D|\xi|)^T D \Omega_1(\xi) x, \, x^T (D|\xi|)^T D \Omega_2(\xi) x\right), \nu \right> = \left< x, D|\xi| \right> 
        \left< 
        \begin{pmatrix}
        \langle D\Omega_1(\xi), x \rangle \\
        \langle D\Omega_2(\xi), x \rangle 
        \end{pmatrix},
        \nu \right>.
    \end{align}
    
    Let us look at the second inner product above: we may write $\left(\langle D\Omega_1(\xi), x \rangle ,\langle D\Omega_2(\xi), x \rangle \right)^T$ as $
        D \Omega(\xi) \cdot x$.
    Then recall Remark \ref{remark:SYM_rm1} (and Notation \ref{notation:perp}): since $D\Omega(\xi): T_{\xi} \mathbb{S}^1 \to T_{\Omega(\xi)} \mathbb{S}^1$, we see that $
        D\Omega(\xi) \cdot x = D \Omega(\xi) \cdot \frac{\xi^\perp}{|\xi|} \left< \xi, e_x^\perp\right> \frac{|x|}{|\xi|}$, where $e_x = x/|x|$; thus, 
    \begin{align} \label{eq:SYM_bound_on_der}
        \av{\left< 
        \begin{pmatrix}
        \langle D\Omega_1(\xi), x \rangle \\
        \langle D\Omega_2(\xi), x \rangle 
        \end{pmatrix},
        \nu \right>} \leq \av{\left<\xi, e_x^\perp\right>} \frac{|x|}{|y|^2} = \frac{|x|}{|y|^2} \dist(\xi, L_Q),
    \end{align}
    recalling that $|D\Omega(\xi)| \leq \frac{1}{|\xi|}$.
    On the other hand, as far as the first inner product in the right hand side of \eqref{eq:SYM_ErrorB_1} is concerned, we immediately see that it's bounded above by $|x|$. Thus 
    \begin{align}
        \left| \eqref{eq:SYM_ErrorB_1} \right| \leq \frac{|x|^2}{|y|^2} \dist(\xi, L_Q). 
    \end{align}
    As $\xi \in [\xi_{0, x}, y]$, we also have that $\dist(\xi, L_Q) \leq \dist(y, L_Q)$. We therefore conclude that 
    \begin{align*}
        \frac{1}{r} \int \av{ \frac{\left<  II, \nu\right> }{r} }\, \phi\ps{\av{\frac{y}{r}}^2} \, d \mu(y)& \lesssim \frac{1}{r} \int \frac{ |\left<x, D(\xi)\right>| \, |\left< D \Omega(\xi) x, \nu \right> | }{r} \phi\ps{\av{\frac{y}{r}}^2} \, d \mu(y) \\
        & \lesssim \frac{|x|^2}{r^4} \int_{B(0,r)} \dist(y, L_Q) \, d \mu(y).
    \end{align*}
 
\subsubsection{Bounds for $III$} 
Let us now look at 
\begin{align} \label{eq:GK_A3_3}
    & \av{\frac{1}{r} \int \frac{\ip{III, \nu}}{r} \, \phi \ps{\av{\frac{y}{r}}^2} \, d\mu(y)} \nonumber \\
    & = \av{ \frac{1}{r} \int \frac{ \ip{\ps{x^T |\xi| D^2\Re \Omega(\xi)x, \, x^T |\xi| D^2 \Im \Omega(\xi) x}^T, \, \nu }}{r} \phi \ps{\av{\frac{y}{r}}^2}\, d\mu(y)}.
\end{align}

To estimate this, we have to resort to (even more boring) computations. Apologies for any inconvenience. For this part, we will distinguish between real and imaginary part, rather than using the indices $1$ and $2$; also, we will do the computations using $y$ as variable (instead of $\xi$), to make the notation less cumbersome.

Recall that
\begin{align}
    D^2\Re \Omega(y) = \begin{pmatrix}
    \partial_1^2 \cos(\Omega(\arg(y))) & \partial_1 \partial_2 \cos(\Omega(\arg(y))) \\
    \partial_2 \partial_1 \cos(\Omega(\arg(y))) & \partial_2^2 \cos(\Omega(\arg(y)))
    \end{pmatrix}
\end{align}
The same holds for $D^2\Im \Omega(y)$ when we replace $\cos$ with $\sin$. We compute
\begin{align*}
    \partial_1^2 \left( \cos(\Omega(\arg(y))) \right) & = \left((D^2 \cos)(\Omega(\arg(y))) \right)\, \left[ \Omega'(\arg(y)) \, \partial_1 \arg(y) \right]^2 \\
    & + (D \cos(\Omega(\arg(y))))  \Omega''(\arg(y))\left( \partial_1\arg(y)\right)^2 \\
    & + (D \cos(\Omega(\arg(y))))  \Omega'(\arg(y)) \partial_1^2\arg(y).
\end{align*}
The same holds for $\partial_2^2 \cos(\Omega(\arg(y)))$ if we replace  $\partial_1$ with $\partial_2$.
We also have the mixed derivatives
\begin{align*}
    \partial_1 \partial_2 \cos(\Omega(\arg(y))) & = \left((D^2 \cos)(\Omega(\arg(y))) \right) \left[ \Omega'(\arg(y)) \left( \partial_1\arg(y)\right) \left( \partial_2\arg(y) \right) \right] \\
    & + \left( (D \cos) (\Omega(\arg(y))) \right) \Omega''(\arg(y)) \partial_1 \arg(y) \partial_2\arg(y) \\
    & + \left( (D \cos) (\Omega(\arg(y))) \right) \Omega'(\arg(y)) \partial_1\partial_2\arg(y).
\end{align*}
Clearly the same calculations hold when computing $D^2 \Im \Omega(y)$: we replace $\cos$ with $\sin$. 
Now we split the matrix $D^2 \Re \Omega(y)$ into three matrices, corresponding to the three terms in the sum above. We denote the first one as $M^\Re_1$, the second one as $M^\Re_2$ and the third one as $M^\Re_3$; we will denote the corresponding matrices for $\Im \Omega(y)$ by $M^\Im_i$, $i=1,2,3$. 
Thus we may split the integral in \eqref{eq:GK_A3_3} as 
\begin{align*}
    & \sum_{i=1}^3 \frac{1}{r} \int \frac{ \left< \begin{pmatrix} 
    x^T M^\Re_i x \\
    x^T M^\Im_i x 
    \end{pmatrix}
    , \nu \right>
    }{r} 
    \phi \ps{\av{\frac{y}{r}}^2} \, d\mu(y) \\
    & =:A_{3,1} + A_{3,2} + A_{3,3}.
\end{align*}

\underline{Estimates for $A_{3,1}$.}
Let us introduce the following notation.
\begin{align*}
    & [11]_1 := \left[ \Omega'(\arg(y)) \, \partial_1 \arg(y) \right]^2 \\
    & [12]_1 := \left[ \Omega'(\arg(y)) \left( \partial_1\arg(y)\right) \left( \partial_2\arg(y) \right) \right] =: [21]_1\\
    & [22]_1 := \left[ \Omega'(\arg(y)) \, \partial_2 \arg(y) \right]^2.
\end{align*}
Then we can write 
\begin{align*}
    M^\Re_1 = \begin{pmatrix}
    D^2\cos(\hdots)[11]_1 & D^2 \cos( \hdots)[12]_1 \\
    D^2 \cos(\hdots) [21]_1 & D^2 \cos( \hdots) [22]_1
    \end{pmatrix}
    '
\end{align*}
where the dots stand for $\Omega(\arg(y))$. 
We compute:
\begin{align*}
  \left< 
  \begin{pmatrix}
  x^T M^\Re_1 x \\
  x^T M^\Im_1 x 
  \end{pmatrix}
  , \nu \right> & = -x_1^2 [11]_1 \left( \cos(\hdots) \nu_1 + \sin(\hdots) \nu_2 \right) \\
  & -2x_1 x_2 [12]_1 \left( \cos(\hdots) \nu_1 + \sin(\hdots) \nu_2 \right) \\
  & - x_2^2 [22]_1 \left( \cos(\hdots) \nu_1 + \sin(\hdots) \nu_2\right)\\
  & = - \left< \Omega(y), \nu \right> \left( x_1^2[11]_1 + 2x_1x_2 [12]_1 + x_2^2 [22]_1\right).
\end{align*}
Now, because
\begin{align*}
    \left| x_1^2[11]_1 + 2x_1x_2 [12]_1 + x_2^2 [22]_1\right|  \lesssim \frac{|x|^2}{|y|^2},
\end{align*}
we see that
\begin{align*}
    \av{\frac{1}{r} \int |y| \frac{ \left< \begin{pmatrix} 
    x^T M^\Re_1 x \\
    x^T M^\Im_1 x 
    \end{pmatrix}
    , \nu \right>
    }{r} 
    \phi \ps{\av{\frac{y}{r}}^2} \, d\mu(y)}
    \lesssim \frac{|x|^2}{r^4} \int_{B(0, r)} \dist(y, L_Q) \, d\mu(y),
\end{align*}
where we used again that $\dist(\xi, L_Q) \leq \dist(y, L_Q)$.  

\underline{Estimates for $A_{3,2}$.} Let us write
\begin{align*}
    & [11]_2 :=\Omega''(\arg(y)) \left( \partial_1 \arg(y)\right)^2 \\
    & [12]_2 :=  \Omega''(\arg(y))  \partial_1 \arg(y) \partial_2\arg(y)=:[21]_2 \\
    & [22]_2 :=  \Omega''(\arg(y)) (\partial_2 \arg(y))^2.
\end{align*}
We have
\begin{align*}
    M^\Re_2 = \begin{pmatrix}
    D \cos( \hdots) [11]_2 & D \cos( \hdots) [12]_2 \\
    D \cos(\hdots) [21]_2 & D \cos (\hdots) [22]_2
    \end{pmatrix}.
\end{align*}
As before, we write out $\left< (x^T M^\Re_2 x, x^T M^\Im_2 x), \nu \right>$ to see that it equals to
\begin{align*}
    & x_1^2 [11]_2  \left( D \cos(\hdots) \nu_1 + D \sin (\hdots)  \nu_2 \right) \\
   &  +  x_2^2 [22]_2 \left( D \cos(\hdots) \nu_1 + D \sin(\hdots)\nu_1\right) \\
   & + 2 x_1 x_2 [12]_2 \left( D \cos (\hdots) \nu_1 + D \sin(\hdots) \nu_2 \right).
\end{align*}
Notice that
\begin{align*}
    [11]_2= \Omega''(\arg(y)) (\partial_1 \arg(y))^2 = \Omega'(y) \frac{\Omega''(\arg(y))}{\Omega(\arg(y))} \partial_1(\arg(y))^2.
\end{align*}
For all $y$, we see that 
\begin{align*}
\frac{\Omega''(\arg(y))}{\Omega'(\arg(y))} \leq C,
\end{align*}
for some universal constant $C>0$. Indeed, because $\Omega$ is bi-Lipschitz, we have that $\Omega'(y) \leq \|\Omega\|_{\mathrm{bi-Lip}}$. Moreover, $\Omega''$ is continuous on a compact subset of the real line, thus has a maximum.
Then we may write
\begin{align*}
    \left< \left( x^T M^\Re_2 x, x^T M^\Im_2 x \right) , \nu \right> & = x_1 \frac{\Omega''(\arg y)}{\Omega'(\arg y)} \partial_1 \arg(y) \, x_1 \left( \partial_1 \cos(\hdots) \nu_1 + \partial_1 \sin(\hdots) \nu_2 \right) \\
    & + x_2 \frac{\Omega''(\arg y)}{\Omega'(\arg y)} \partial_2 \arg(y) \, x_2 \left( \partial_2 \cos(\hdots) \nu_1 + \partial_2 \sin(\hdots) \nu_2 \right) \\
    & + x_1 \frac{\Omega''(\arg y)}{\Omega'(\arg y)} \partial_1 \arg(y) \, x_2 \left( \partial_2 \cos (\hdots) \nu_1 + \partial_2 \sin(\hdots) \, \nu_2 \right) \\
    & + x_2 \frac{\Omega''(\arg y)}{\Omega'(\arg y)} \partial_2 \arg(y) \, x_1 \left( \partial_1 \cos(\hdots) \nu_1 + \partial_1 \sin(\hdots) \nu_2 \right) \\
    & = \left< D\Omega(y)\cdot x', \nu \right> + \left< D \Omega (y) \cdot x'', \nu \right>,
\end{align*}
where 
\begin{align*}
    x' = \begin{pmatrix}
    x_1 \, \left( x_1 \frac{\Omega''(\arg y)}{\Omega'(\arg y)} \partial_1 \arg(y) \right) \\
    x_2 \, \left(x_2 \frac{\Omega''(\arg y)}{\Omega'(\arg y)} \partial_2 \arg(y)\right)
    \end{pmatrix}
\end{align*}
and
\begin{align*}
    x'' = 
    \begin{pmatrix}
    x_1 \left(x_2 \frac{\Omega''(\arg y)}{\Omega'(\arg y)} \partial_2 \arg(y)\right) \\
     x_2 \left( x_1 \frac{\Omega''(\arg y)}{\Omega'(\arg y)} \partial_1 \arg(y)\right)
     \end{pmatrix}.
\end{align*}

We see first that $\partial_2 \arg y = \frac{y_1}{|y|^2}$ and that $\partial_1 \arg y= \frac{-y_2}{|y|^2}$. Thus we have that $(x')_1 = - x_1 x_1 (-y_2 )\frac{\Omega''(\arg y)}{|y|^2 \Omega'(\arg y)}$. By Taylor's theorem, we have that
\begin{align*}
    & y_1 = \frac{|y|}{|x|}x_1 - |y| \sin(\zeta_1)( \theta_y - \theta_x) \\
    & y_2 = \frac{|y|}{|x|}x_2 + |y| \cos(\zeta_2)(\theta_y - \theta_x),
\end{align*}
where $\zeta_1, \zeta_2 \in [\theta_y, \theta_x]$. 
Hence we may write 
\begin{align*}
    x' = \frac{1}{|y|^2}\begin{pmatrix}
    x_1 \left(x_1 (-x_2) \frac{|y|}{|x|} \frac{\Omega''(\arg y)}{\Omega'(\arg y)} \right)\\
    x_2 \left( x_2 x_1 \frac{|y|}{|x|} \frac{\Omega''(\arg y)}{\Omega'(\arg y)} \right)
    \end{pmatrix}
    + 
    \frac{1}{|y|^2}\begin{pmatrix}
    x_1 \left(x_1 |y| \sin(\zeta_1) (\theta_y-\theta_x)\frac{\Omega''(\arg y)}{\Omega'(\arg y)} \right) \\
    x_2 \left(x_2 |y| \cos(\zeta_2) (\theta_y-\theta_x)\frac{\Omega''(\arg y)}{\Omega'(\arg y)} \right)
    \end{pmatrix}.
\end{align*}
And also we have
\begin{align*}
    x'' = \frac{1}{|y|^2}\begin{pmatrix}
    x_1 \left( x_2 x_1 \frac{|y|}{|x|} \frac{\Omega''(\arg y)}{\Omega'(\arg y)} \right) \\
    x_2 \left( x_1 (-x_2) \frac{|y|}{|x|} \frac{\Omega''(\arg y)}{\Omega'(\arg y)} \right)
    \end{pmatrix}
    + 
   \frac{1}{|y|^2} \begin{pmatrix}
    x_1 \left(x_2 |y| \cos(\zeta_1) (\theta_y-\theta_x)\frac{\Omega''(\arg y)}{\Omega'(\arg y)} \right) \\
    - x_2 \left(x_2 |y| \sin(\zeta_2) (\theta_y - \theta_x)\frac{\Omega''(\arg y)}{\Omega'(\arg y)} \right)
    \end{pmatrix}
\end{align*}
Note that
\begin{align*}
    |y| |\theta_y- \theta_x| \lesssim \dist(y, L_Q).
\end{align*}
Indeed, $|\theta_y-\theta_x|^2 \sim \sin(|\theta_y-\theta_x|)^2 + \sin(|\theta_y-\theta_x|/2)^4 \leq 2 \sin(|\theta_y-\theta_x|)^2$.
Recall that $|y| |D\Omega(y)| \lesssim 1$. Thus
\begin{align*}
    & \av{ \frac{1}{r} \int |y|\frac{\left< \left( x^T M^\Re_2 x, x^T M^\Im_2 x \right) , \nu \right>}{r} \phi \ps{\av{\frac{y}{r}}^2} \, d\mu(y) }\\
    & \lesssim \frac{1}{r^2} \int |y|\frac{\Omega''(\arg y)}{|y|^2 \Omega'(\arg y)} |D \Omega(y)| |x|^2 \dist(y, L_Q) \phi \ps{\av{\frac{y}{r}}^2} \, d\mu(y) \\
    & \leq C \frac{|x|^2}{r^4} \int_{B(0,r)} \dist(y, L_Q)\, d\mu(y).
\end{align*}

\underline{Estimates for $A_{3,3}$}.
We see that we may re write $\left< \left(x^T M_3^\Re x, x^T M^\Im_3 x\right), \nu \right>$ as 
\begin{align*}
    & \left( D \cos (\hdots) \nu_1 + D \sin(\hdots) \nu_2 \right) \Omega'(\arg y) |y|^{-4} \\
    & \times \left[ (x_1^2 (2 y_1 y_2) - 2 x_1 x_2 y^2_1) + (x_2^2 (-2y_1 y_2) + 2x_1 x_2 y_2^2\right] \\
    & =: \left( \hdots \right) \times [\mathcal{A} + \mathcal{B}].
\end{align*}
If we expand as above $y_1$ and $y_2$ in terms of $x_1 $ and $x_2$ respectively, we obtain that
\begin{align*}
    \mathcal{A} & = x_1^2 \frac{|y|^2}{|x|} x_2 \cos(\zeta)(\theta_x - \theta_y) - x_1^2 \frac{|y|^2}{|x|} x_2 \sin(\zeta)(\theta_x - \theta_y) - x_1^2 |y|^2 \sin(\xi) \cos(\zeta) (\theta_x - \theta_y)^2\\
    & + 4 x_1 x_2 \frac{|y|^2}{|x|}x_1 \sin(\zeta) (\theta_x - \theta_y) - 2 x_1 x_2 |y|^2 \sin(\zeta)^2 (\theta_x - \theta_y)^2 =: \sum_{j=1}^5 \mathcal{A}_i.
\end{align*}
It is immediate to see that $\mathcal{B}$ has the very same structure. Notice that for $i=1,2,4$ we have that $|\mathcal{A}_i|, |\mathcal{B}_i| \lesssim |y||x|^2 \dist(y, L_Q)$; on the other hand, for $i=3,5$, we have that $|\mathcal{A}_i|,|\mathcal{B}_i|\lesssim |x|^2 \dist(y,L_Q)^2 \lesssim |y||x|^2 \dist(y, L_Q)$.
Thus 
\begin{align*}
    & \frac{1}{r^2}\int_{B(0,r)} |y|\av{\left( D \cos (\hdots) \nu_1 + D \sin(\hdots) \nu_2 \right) \Omega'(\arg y) |y|^{-4} }|y||x|^2 \dist(y, L_Q) \, d \mu(y) \\
     & \lesssim \frac{|x|^2}{r^4} \int_{B(0,r)} \dist(y, L_Q) \, d\mu(y).
\end{align*}
This shows the desired bound for $A_{3,3}$ and so for $A_3$. 

\subsubsection{Estimates on $B_{1,1}$}
Recall that 
\begin{align*}
    B_{1,1}(x) = \frac{1}{r} \int \frac{K(-y)}{r}\, \phi' \ps{\av{\frac{y}{r}}^2} \, \left[ - \av{\frac{DK(-y) \cdot x + x^T DK(\xi) x}{r}}^2 \right]\, d \mu(y). 
\end{align*}
Let us estimate $\left< B_{1,1}(x), \nu \right>$; it is immediate from Lemma \ref{lemma:SYM_dotprods} that $|\left< K(-y), \nu\right>| \sim \dist(y, L_Q)$. Moreover, 
\begin{align} \label{eq:GK_estSO}
   \av{\frac{DK(-y) \cdot x + x^T D^2K(\xi) x}{r}}^2  \lesssim \frac{1}{r^2}\left(|x|^2 + \frac{|x|^4}{|y|^2}\right)  \lesssim \frac{|x|^2}{r^2}.
\end{align}
Then we see that 
\begin{align*}
    \av{ \left< B_{1,1}(x), \nu \right>}& \lesssim \frac{1}{r} \int \frac{\dist(y, L_{Q})}{r} \, \phi \ps{\av{\frac{y}{r}}^2} \, \frac{|x|^2}{r^2} \, d\mu(y) \\
    & \lesssim \frac{|x|^2}{r^4} \int_{B(0, r)} \dist(y, L_{Q}) \, d\mu(y). 
\end{align*}

\subsubsection{Estimates on $B_{1,2,2}$}
We want to compute 
\begin{align*}
    \av{\left< B_{1,2,2}(x), \nu\right> } = \av{\frac{1}{r} \int \frac{\left<K(-y), \nu \right>}{r} \phi' \ps{\av{\frac{y}{r}}^2} \, \left[ \left< \frac{K(-y)}{r}, \, \frac{x^T D^2K(\xi) x}{r} \right> \right] \, d \mu(y)}.
\end{align*}
Again, $\av{\left< K(-y), \nu\right> } \sim \dist(y, L_Q)$. On the other hand, we see that
\begin{align} \label{eq:GK_estDP}
    \frac{1}{r^2}\av{\left< K(-y), x^T D^2K(\xi) x\right>} & \lesssim \frac{1}{r^2} \ps{ |y||x|^2 |y|^{-1} } = \frac{|x|^2}{r^2}.
\end{align}
Hence we obtain that
\begin{align*}
    \av{\left< B_{1,2,2}(x), \nu\right> } \lesssim \frac{|x|^4}{r^6} \int_{B(0,r)} \dist(y, L_Q) \, d\mu(y) \lesssim \frac{|x|^2}{r^4} \int_{B(0,r)} \dist(y, L_Q) \, d\mu(y).
\end{align*}

\subsubsection{Estimates for $B_2$}
We want to compute $\av{\left<B_2(x), \nu \right>}$, that is
\begin{align*}
    & \frac{1}{r} \int \frac{\left<D K(-y) \cdot x, \nu \right>}{r}  \phi'\ps{\av{\frac{y}{r}}^2} \, \left[ SO\right] \, d\mu(y) +  \frac{1}{r} \int \frac{\left< D K(-y) \cdot x, \nu \right>}{r}  \phi'\ps{\av{\frac{y}{r}}^2} \left[ DP \right] \, d\mu(y) \\
    & := B_{2,1}(x) + B_{2,2}(x). 
\end{align*}
We first estimate the common term $\left< DK(-y) \cdot x, \nu \right>$. As before, we write it explicitly as 
\begin{align*}
    \left< D(|y|) \Omega(-y) \cdot x, \nu \right> + \left< |y|D\Omega(-y)\cdot x, \nu \right>.
\end{align*}
On one hand, we see that
\begin{align} \label{eq:GK_B21a}
    \left<D|y| \Omega(-y) \cdot x, \nu \right> = \left< D |y|, x \right>\left< \Omega(-y), \nu \right>.
\end{align}
Recall that, by the way $\nu$ was defined and Lemma \ref{lemma:SYM_dotprods}, $|\left< \Omega(y), \nu \right>| \sim |y|^{-1} \dist(y, L_Q)$. Moreover, 
\begin{align}\label{eq:GK_B21c}
    |\left< D|y|, x \right>| \lesssim |x|.
\end{align}

On the other hand, arguing as in \eqref{eq:SYM_bound_on_der},   $D\Omega(y) \cdot x= D \Omega(y) \cdot \frac{y^\perp}{|y|} \frac{|x|}{|y|}\left< y, e^\perp\right>$; and so 
\begin{align} \label{eq:GK_B21b}
    \av{\left< |y| D\Omega(-y) \cdot x, \nu \right>} = \frac{|x|}{|y|}\av{\left<y, e^\perp\right>} \lesssim \frac{|x|}{|y|} \dist(y, L_Q).
\end{align}
Putting together \eqref{eq:GK_B21a} and \eqref{eq:GK_B21c} for one term, and \eqref{eq:GK_B21b} for the other, we see that
\begin{align}
    \av{\left< DK(-y)\cdot x, \nu \right>} \lesssim \dist(y, L_Q). 
\end{align}
Thus: estimates \eqref{eq:GK_estSO} and \eqref{eq:GK_estDP} of the term $SO$ and $DP$, respectively, let us conclude that
\begin{align} \label{eq:GK_boundB2}
    \av{\left< B_{2}(x) ,  \nu \right>} \lesssim \frac{|x|^2}{r^4} \int_{B(0,r)} \dist(y, L_Q) \, d\mu(y).
\end{align}

\subsubsection{Estimates for $B_3$}
This term has the same form as $A_3$, the only difference being the presence of $DP$ and $SO$. However, from \eqref{eq:GK_estSO} and \eqref{eq:GK_estDP}, we see that both are $\leq 1$. Thus we obtain the bound
\begin{align}\label{eq:GK_boundB3}
    |\left< B_3(x) , \nu \right> | \lesssim \frac{|x|^2}{r^4} \int_{B(0,r)} \dist(y, L_Q) \, d\mu(y)
\end{align}
as in Subsection \ref{subsection:GK_A3}.

\subsubsection{Estimates for $C$}
 We Taylor expand $K(x-y)$ as before and split up $C(x)$ consequently so that
 \begin{align*}
     & C_1(x) = \frac{1}{r} \int \frac{K(-y)}{r} \phi''(\xi_{s_0,s}) [DP + SO]^2 d\mu(y)\\
     & C_2(x) = \frac{1}{r} \int \frac{DK(-y)}{r} \phi''(\xi_{s_0,s}) [DP + SO]^2 d\mu(y)\\
     & C_3(x) = \frac{1}{r} \int \frac{x^T D^2 K(\xi_{0,x}-y) x}{r} \phi''(\xi_{s_0,s}) [DP + SO ]^2 \, d\mu(y).
 \end{align*}
 The proofs that we gave for the previous terms hold for these ones, too. Hence we have the bound
 \begin{align} \label{eq:GK_boundC}
     |\left< C(x), \nu \right> | \lesssim \frac{|x|^2}{r^4} \int_{B(0,r)} \dist(y, L_Q) \, d\mu(y),
 \end{align}
 These estimates together prove Lemma \ref{lemma:GK_errorx}.
 
 \subsubsection{A further estimate on the error term}
 We now want to prove a bound on $E$ when evaluated at any point in $3Q$ (not just at a balanced point).
 \begin{lemma}
 Keep the notation as above; in particular $z \in 3Q$, $x_0, x_1$ are balanced points and $L_Q$ is the balanced line. Then 
 \begin{align} \label{lemma:GK_errorz}
     |\left< E(z), \nu \right>| \lesssim \frac{|z|^2}{r^4} \int_{B(x_0,r)} \dist(y, L_Q) \, d\mu(y) + \frac{1}{A^2 r}\dist(z, L_{Q}). 
 \end{align}
 \end{lemma}
 \begin{proof}
 Again, we assume $x_0=0$.
 The proof of this lemma is very similar to the one for Lemma \ref{lemma:GK_errorx}. Indeed, for the terms $B_{1,1}$, $B_{1,2,2}, C_1$ the proof goes through verbatim, since we only used that $|x| \leq r$, and the same holds for $|z|$ (recall that $r \in [A\ell(Q), 2A \ell(A)]$, and $A$ is a large constant).
 
On the other hand, let us consider the term $\left< B_{2}(z), \nu \right>$:
\begin{align*}
    &\frac{1}{r} \int \frac{\left<D K(-y) \cdot z, \nu \right>}{r} \phi' \ps{ \av{\frac{y}{r}}^2}[SO] \, d \mu(y)\\
    & = \frac{1}{r} \int \frac{\left<(D |y|) \Omega(-y)\cdot z, \nu \right>}{r} \phi' \ps{\av{\frac{y}{r}}^2} \,[SO] d\mu(y) \\
    & + \frac{1}{r} \int \frac{\left< |y|D\Omega(y) \cdot z, \nu \right>}{r} \phi' \ps{\av{\frac{y}{r}}^2} [SO]\, d\mu(y).
\end{align*}
Now the first term is easily taken care of, as $\left< D|y| \Omega(y) \cdot z, \nu \right> = \left< D |y|, z \right>\left< \Omega(y), \nu \right>$.
On the other hand, we have that $D \Omega(y) \cdot z = D \Omega(y) \cdot z^{\perp(y)}$. Denote by $\tilde z$ the projection of $z$ onto $L_Q$. We see that $|z^{\perp(y)}| \leq |(z- \tilde z)^\perp| + |(\tilde z)^\perp|$. Now, it is clear that $|(z-\tilde z)^\perp| \leq |z- \tilde z| = \dist(z, L_Q)$. But also, $|(\tilde z)^\perp| \lesssim |x^\perp|$ since $z \in 3Q$. Moreover, as in \eqref{eq:GK_B21b}, we have that $|x^\perp| \lesssim \dist(y, L_Q)$. With these consideration, and recalling that $|SO| \lesssim |x|^2 r^{-2}$ (see \eqref{eq:GK_estSO}), we obtain the bound
\begin{align*}
\av{ \frac{1}{r} \int \frac{ \left< |y|D \Omega(y) \cdot z, \nu \right> }{r} \phi' \ps{\av{ \frac{y}{r}}^2} \,[SO]d\mu(y) }  & \lesssim  \frac{|z|^2}{r^4} \int_{B(0,r)} \dist(y, L_Q) \, d\mu(y)\\
& + \frac{1}{A^2 r} \dist(z, L_Q), 
\end{align*}
where in the last term we used the AD-regularity of $\mu$.

The proofs for the term $\left<A_3(z), \nu\right>$ and $\left<B_3(z), \nu \right>$ are just the same as for the terms $\left< A_3(x), \nu\right>$ and $\left< B_3(x), \nu\right>$. Notice, however, that to carry out the computations, we need to assume that $|z| \neq 0$. This can be done without loss of generality: $\mu$ is ADR, thus $\mu(\{z\})=0$. Finally, the term $\left< C(z) , \nu \right>$ may be split into $C_1$, $C_2$ and $C_3$; these ones may be dealt with as in the previous sections. 
\end{proof}

\begin{lemma}
For $z \in 3Q$, we have  
\begin{align}
   \frac{\dist(z, L_{Q})}{r} \lesssim \frac{\ell(Q)^2}{r^4} \int_{B(x_0, r)} \dist(y, L_Q) \, d\mu(y).
\end{align}
\end{lemma}
\begin{proof}
Since $\mu$ is an $\Omega$-symmetric measure and $0, x \in \spt(\mu)$, we have that
\begin{align*}
    0= C_{\Omega, \phi}(0, r) - C_{\Omega,\phi}(x, r) = T(x) + E(x), 
\end{align*}
thus
\begin{align} \label{eq:GK_errT}
    - T(x) = E(x). 
\end{align}
Now, for $z \in  3Q$,
\begin{align*}
    \left< T(e_z), \nu \right> & = \left< T \ps{ \frac{z-\tilde z}{|z - \tilde z|}}, \nu \right>\\
    & = \frac{1}{\dist(z, L_Q)} \left< T(z - \tilde z), \nu \right> \\
    & = \frac{1}{\dist(z, L_Q)} \left< T(z) - T(\tilde z), \nu \right>.
\end{align*}
Because $\tilde z \in L_Q$, and $\frac{x}{|x|}$ forms a basis for $L_Q$ we can write it as $\tilde z= \alpha \frac{x}{|x|}$; by the linearity of $T$ we then have that $T(\tilde z)= \frac{\alpha}{|x|} T(x)$, and, by \eqref{eq:GK_errT}, $\left<T(\tilde z), \nu\right>= \frac{\alpha}{|x|} \left< -E(x), \nu \right>$. Notice in passing that $\frac{|\alpha|}{|x|} \lesssim 1$, since $z \in 3Q$. Thus we see that
\begin{align*}
    - \left< T(e_z), \nu \right> = \frac{1}{\dist(y, L_Q)} \left( - \left<E(z), \nu\right> + \frac{\alpha}{|x|}\left< E(x), \nu\right> \right).
\end{align*}
By Lemma \ref{lemma:SYM_Tlowerbound}, we see that $-\left< T(e_z), \nu\right> \gtrsim \frac{\delta_0^2}{r}$. Thus we have
\begin{align*}
    \frac{\delta_0^2}{r} \lesssim \frac{1}{\dist(y, L_Q)} \left( - \left<E(z), \nu\right> + \frac{\alpha}{|x|}\left< E(x), \nu\right> \right).
\end{align*}
Now we may take the absolute value of the right hand side of this inequality, and we apply the bounds proved for the error terms:
\begin{align*}
    \frac{1}{r} \lesssim \frac{1}{\dist(z, L_{Q})} \left(\frac{|x|^2}{r^4} \int_{B(0, r)} \dist(y, L_{Q}) \, d\mu(y) + \frac{1}{r} A^{-2} \dist(z, L_{Q})\right).
\end{align*}
As $A\geq 2$, we finally obtain
\begin{align*}
    \frac{\dist(z, L_Q)}{2r} \leq \frac{\dist(z, L_Q)}{r}(1-A^{-2}) \lesssim  \frac{\ell(Q)^2}{r^4} \int_{B(0, r)} \dist(y, L_{Q}) \, d\mu(y).
\end{align*}
\end{proof}
 
\begin{lemma} \label{lemma:GK_squaredist}
Keep the notation as above (in particular $z \in 3Q$ is fixed and $N \sim \log(A)$). Then 
\begin{align}
    \left(\frac{\dist(z, L_{Q})}{r}\right)^2 \lesssim \frac{\ell(Q)^2}{r^2} \log(A) \sum_{k=0}^N \beta_{\mu, 2}(x_0, 2^k \ell(Q))^2. 
\end{align}
\end{lemma}
\begin{proof}
Let $x_0 \in F_0 \cap G_0$, as we defined in the proof of Lemma \ref{lemma:GK_goodpoints} and let us denote by $P(Q)$ the line which minimises $\beta_{\mu, 2}(Q)$; then we see that 
\begin{align*}
    \dist(y, L_{Q}) \leq \dist(y, P(x_0, r)) + \dist_H \left(P(x_0, r) \cap B(x_0, r), L_{Q} \cap B(x_0, r)\right).
\end{align*}
This, together with the assumption that $x_0$ belongs to $F_0$, let us conclude that 
\begin{align}
    \dist(y, L_{Q}) \lesssim r \sum_{k=0}^N \beta_{\mu, 2}(x_0, 2^k \ell(Q)),
\end{align}
where $N \sim \log(A)$. Hence we deduce that 
\begin{align*}
    \frac{1}{r} \int_{B(x_0,r)} \left( \frac{\dist(y, L_{Q})}{r} \right)^2 \, d\mu(y) & \lesssim \frac{1}{r} \int_{B(x_0, r)} \ps{ \frac{ \dist(y, L_{Q})}{r}}^2 d\mu(y) \\
    & + \frac{1}{r}\int_{B(x_0,r)} \ps{ \sum_{k=0}^N \beta_{\mu, 2} (x_0, 2^k \ell(Q)) }^2 d\mu(y)\\
    & \lesssim c_0\log(A)  \sum_{k=0}^N \beta_{\mu, 2} (x_0, 2^k \ell(Q))^2.
\end{align*}
\end{proof}





==> 10_Lip_estimate.tex <==
\section{Estimates on Lipschitz graphs with small constant}

In \cite{tolsa07}, Tolsa proved the following.
\begin{theorem}[\cite{tolsa07}, Theorem 1.3]
Consider an $n$-dimensional Lipshitz graph $\Gamma$...
\end{theorem}

Our aim here is to prove the same theorem for the class of kernels we have considered so far. 

\subsection{Upper estimate}
\begin{lemma}
Same assumptions as in Lemma 3.1 of \cite{tolsa07}. Then
\begin{align*}
    \|\mbox{p.v.} T\mu \|_{L^2(\mu)}^2 \lesssim \sum_{Q \in \mucubes}  \alpha(Q)^2 \mu(Q). 
\end{align*}
\end

\subsection{Lower estimates}
\begin{lemma}
Same assumptions as above. Then we have that
\begin{align*}
    \|\mbox{p.v.}T \mu\| \gtrsim 
\end{align*}
\end{lemma}


==> 999_scarti.tex <==
\section{Lettera}
Le mie gioie giornaliere sono: ho accertato che la mia dimostrazione sia corretta; ho finalmente intuito il modo per proseguire l'argomentazione: un superficie piana viene mappata ad una superficie che puo' essere considerata una perturbazione di un piano da una mappa Lipschitz \textit{con constante piccola} -  questo semplice fatto si dimostra fondamentale nell'applicazione del mio metodo; quest'altro progetto, di natura topologica, sembra procedere bene. 
Come ti posso spiegare la mia vita degli ultimi due anni? Non sbagliarti: non e' vanto il mio; e' piuttosto rassegnazione - non poter condividere quei puntini di gioia che si generano e muoiono, quasi in maniera casuale, durante la giornata. La gioiosa ebbrezza rimane in me; quindi si dissolve rapidamente; evaporando al mio respiro, si disperde tra i miei pensieri: mai concreta, mai attuata nel linguaggio; mai percepita da altri che me - mai esistita. Eppure, come lucciole, io li sento questi momenti, e ne sono sempre grato; ti scrivo per parlartene; in realta': ti voglio parlare, e basta. 
Non sono bravo a raccontare storie; quindi non ti raccontero' di me; dopotutto, che importanza ha per te? E non ha alcuna importanza per me. Cio' che mi importa, cio' che voglio, e' di lasciar correre sulla tastiera le dita,  di lasciar libero il flusso tra le mie mani e la coscienza: tu sei sempre stata il .... per scatenare la reazione; ma devo e voglio rivolgermi a te, per continuarla e sostenerla, questa reazione. Mi viene in mente: da poco ci eravamo lasciati. Ma io ti pensavo, ti pensavo; ti volevo indietro: ti telefonai. Ricordo la sorpresa di poter essere sincero; di poter parlare senza dover spiegare, modificare il mio pensiero, creare una narrativa parallela al mio sentimento: non c'era una audience, da soddisfare, in qualche modo, all'altro capo; c'era. Ebbene chi?; una voce: una mano che faceva correre le sue cinque dita tra i miei capelli, e una presenza che assorbiva, assorbiva quello che dicevo, e si mostrava sensibile al preciso significato - oppure, all'opposto, all'insicurezza sul significato, ossia alla scarsa comprensione di me stesso. 

Tutto cio' tu non volevi 'farlo'. Tu sei sempre 'stata', per me, cosi'. Ma non e' amore, questo; ne' tanto meno innamoramento. E' piuttosto la mia, personale, mitologia: la tua figura si origina tra i miei ricordi; ma, per causa oppure effetto, questi ricordi non si collocano con gli altri: terreni questi; si alzano al di sopra, nebbiosi, lontani: sacri. Il mio essere, non io, perche' io non ho avuto parola in merito, mai mi e' stata chiesta un'opinione, una scelta, il mio essere, lui, indipendente, ti ha eletto a figura sacra, immortale, venerata. Ed io non posso che rispettare la sua decisione: ne ammiro, anzi, la saggezza. 

Quindi ti scrivo, cara cosa sacra; e perche' no? Ma ora ho finito gli argomenti; ti cerchero' la prossima volta. 

%%%%%%%%%%%%Arguments from Sublemma \eqref{sublemma:SYMg_lowA2}
With \eqref{e:dot-y-perp}, we have that
    \begin{align*}
        \cos\ps{\ds(\Omega(y),\Omega(e_{x_1}))} \geq \cos \ps{(1+\delta_\Omega)\ds(\hat y, e_x)}
    \end{align*}
    Again, set  $\alpha: =\ds(\hat y, e_{x_1})$. If we Taylor expand the term on the right hand side, we see that
    \begin{align*}
    \cos \ps{(1+\delta_\Omega)\alpha } = \cos\ps{\alpha}- \sin(\xi_{\alpha, \delta_\Omega}) \delta_\Omega\alpha,
    \end{align*}
    where $\xi_{\alpha, \delta_\Omega} \in [\alpha, \alpha(1+ \delta_\Omega)]$. Thus
    \begin{align*}
        \cos\ps{(1+\delta_\Omega)\alpha} \geq \delta_0 - \delta_\Omega \alpha.
    \end{align*}
    Clearly, by our assumption on $\left< y, e_{x_1}\right>$,  $\alpha$ must be less that $ \frac{\pi}{2} - \delta_1$, and therefore we can estimate 
    \begin{align} \label{eq:SYM_posiA}
        \cos\ps{(1+\delta_\Omega) \alpha} \geq \cos(\pi/2- \delta_1) - \delta_\Omega (\pi/2- \delta_1).
    \end{align}
    We would like to have $\cos(\pi/2-\delta_1) - \delta_\Omega(\pi/2-\delta_1) \geq \frac{\cos(\pi/2-\delta_1)}{2}$; this will be the case if 
    \begin{align} \label{eq:SYM_smallLip}
        \delta_\Omega \leq \frac{\cos\ps{\frac{\pi}{2} - \delta_1}}{2\ps{\frac{\pi}{2} - \delta_1}}= \frac{\sin(\delta_1)}{2\ps{\frac{\pi}{2} - \delta_1}}
    \end{align}




Since $\Omega(e_{x_1}) \perp \nu$, we write
\begin{align*}
    \left< \Omega(y), \nu \right> =  \cos(\ds(\hat y, \nu)) =  \sin(\ds(\hat y, \Omega(e_{x_1}))).
\end{align*}
Let us set $\alpha:= d_{\bS}(\hat y, e_{x_1})$. Since $\Omega$ is bi-Lipschitz with constant $1+\delta_\Omega$, we have that
\begin{align}
    \sin(\ds(\Omega(y), \Omega(e_x)) \geq \sin\ps{\alpha(1+\delta_\Omega)^{-1}}.
\end{align}
Taylor expanding $\sin$ around $\alpha$, we obtain 
\begin{align} \label{eq:SYMg_lowA2}
    \sin((1+\delta_\Omega)\alpha)= \sin(\alpha) - \cos(\xi_{\alpha, \delta_\Omega}) \frac{\alpha \delta_\Omega}{1+ \delta_\Omega}.
\end{align}
where $\xi_{\alpha, \delta_\Omega} \in [ (1+\delta_\Omega)^{-1}\alpha, \alpha]$. By \eqref{eq:SYMg_1}, we see that $\delta_1 \leq \alpha \leq \pi/2$, and therefore $0 \leq \cos(\xi_{\alpha, \delta_\Omega}) \leq \cos(\delta_1)$. We want something that looks like 
\begin{align} \label{eq:SYMg_lowA2_2}
    \eqref{eq:SYMg_lowA2} \geq \frac{1}{2} \sin(\alpha):
\end{align} 
if this held, we could conclude that whenever $\left< y, e_z\right> \geq |y| \delta_0$, then also $\left< K(y), \nu \right> \gtrsim |y| \delta_0$. But one can check that \eqref{eq:SYMg_lowA2_2} holds if $\delta_\Omega$ is chosen sufficiently small (say $\delta_\Omega \leq 1/10$). 



 We now look at $\langle II(\xi,x) , \Omega(e_z)\rangle$. 
    To do so, we consider first the term $x\left(D|\xi|\right)^T D \Omega_i (\xi)x^T$. The other one can be dealt with in the same fashion. 
    First, notice that, for $i =1,...,d$, 
    $
        x^T (D|\xi|)^T D\Omega_i(\xi) x = \langle x, D|\xi| \rangle \langle D \Omega_i(\xi) , x \rangle.
    $
    Thus we have that
    \begin{align} \label{eq:SYM_ErrorB_1}
        \left< II(x), \Omega(e_z) \right> = \left< x, D|\xi| \right> 
        \left< 
        \begin{pmatrix}
        \langle \grad\Omega_1(\xi), x \rangle \\
        \vdots \\
        \langle \grad\Omega_d(\xi), x \rangle 
        \end{pmatrix},
        \Omega(e_z) \right>.
    \end{align}
    
    Let us look at the second inner product on the right hand side of \eqref{eq:SYM_ErrorB_1}: we may write $\left(\langle D\Omega_1(\xi),...,x \rangle ,\langle D\Omega_d(\xi), x \rangle \right)^T$ as $
        D \Omega(\xi) \cdot x$.
    Then recall Remark \ref{remark:BT_remdiff} (and Notation \ref{notation:perp}): since $D\Omega(\xi): T_{\xi} \mathbb{S}^{d-1}\to T_{\Omega(\xi)} \mathbb{S}^{d-1}$, we see that $
        D\Omega(\xi) \cdot x = D \Omega(\xi) \cdot \ps{ \sum_{i=1}^{d-1} \xi_i^\perp \left< \xi_i^\perp, e_x\right> |x|}$, where $e_x = x/|x|$; thus, using also \eqref{eq:SYMg_DerK}, 
    \begin{align} \label{eq:SYM_bound_on_der}
        \av{\left< 
        D\Omega(\xi) \cdot x,
        \Omega(e_z)\right>} 
        \lesssim_{\delta_\Omega} \sum_{i=1}^{d-1} \av{ \left< \Omega(\xi_i^\perp), \Omega(e_z) \right>} \av{ \left<\xi_i^\perp, e_x\right> }|x|.
    \end{align}
    Moreover, $|\left< K(\xi_i^\perp), \Omega(e_z)\right>| \sim_{\delta_\Omega} |\left<\xi_i, e_x\right>|$
    recalling that $|D\Omega(\xi)| \leq \frac{1}{|\xi|}$.
    On the other hand, as far as the first inner product in the right hand side of \eqref{eq:SYM_ErrorB_1} is concerned, we immediately see that it's bounded above by $|x|$. Thus 
    \begin{align}
        \left| \eqref{eq:SYM_ErrorB_1} \right| \leq \frac{|x|^2}{|y|^2} \dist(\xi, L_Q). 
    \end{align}
    As $\xi \in [\xi_{0, x}, y]$, we also have that $\dist(\xi, L_Q) \leq \dist(y, L_Q)$. We therefore conclude that 
    \begin{align*}
        \frac{1}{r} \int \av{ \frac{\left<  II, \nu\right> }{r} }\, \phi\ps{\av{\frac{y}{r}}^2} \, d \mu(y)& \lesssim \frac{1}{r} \int \frac{ |\left<x, D(\xi)\right>| \, |\left< D \Omega(\xi) x, \nu \right> | }{r} \phi\ps{\av{\frac{y}{r}}^2} \, d \mu(y) \\
        & \lesssim \frac{|x|^2}{r^4} \int_{B(0,r)} \dist(y, L_Q) \, d \mu(y).
    \end{align*}
    
    
    
    
    
    
    
    
    
    
    
    
    
    
    
    
    
    
    
    
    \iffalse
We want to understand how does the inner products in the image behave with respect to the inner products in the domain. 
 Suppose first that $|y| \geq \left< y, e_x \right> \geq |y|\delta_0$, for $\delta_0$ given by 
    \begin{align} \label{eq:SYM_delte}
        \delta_0 := \cos\left( \frac{\pi}{2} - \delta_1 \right), \delta_1 >0.
    \end{align}
    Then we have that
    \begin{align*}
        \cos\ps{|\Omega(y) - \Omega(e_x)|} \geq \cos \ps{(1+\delta_\Omega)|\arg(y)-\arg(e_x)|}
    \end{align*}
    We will denote by $\alpha= \alpha(y, e_x)= |\theta(y)-\theta(e_x)|$. If we Taylor expand the term on the right hand side, we see that
    \begin{align*}
    \cos \ps{(1+\delta_\Omega)\alpha } = \cos\ps{\alpha}- \sin(\xi) \delta_\Omega\alpha,
    \end{align*}
    where $\xi= \xi(y, e_x)$. Thus
    \begin{align*}
        \cos\ps{(1+\delta_\Omega)\alpha} \geq \delta_0 - \delta_\Omega \alpha.
    \end{align*}
    Clearly, by our assumption on $\left< y, e_x\right>$,  $\alpha$ must be less that $ \frac{\pi}{2} - \delta_1$, and therefore we can estimate 
    \begin{align} \label{eq:SYM_posiA}
        \cos\ps{(1+\delta_\Omega) \alpha} \geq \cos(\pi/2- \delta_1) - \delta_\Omega (\pi/2- \delta_1).
    \end{align}
    We would like to have $\cos(\pi/2-\delta_1) - \delta_\Omega(\pi/2-\delta_1) \geq \frac{\cos(\pi/2-\delta_1)}{2}$; this will be the case if 
    \begin{align} \label{eq:SYM_smallLip}
        \delta_\Omega \leq \frac{\cos\ps{\frac{\pi}{2} - \delta_1}}{2\ps{\frac{\pi}{2} - \delta_1}}= \frac{\sin(\delta_1)}{2\ps{\frac{\pi}{2} - \delta_1}}
    \end{align}

Similarly, if $|y| \geq \left< y, e_z\right> \delta_0 |y|$, the we see that
\begin{align}
    \left< K(y), \Omega(e_z) \right> \geq \frac{\delta_0}{2} \mbox{ if } \delta_\Omega \mbox{ satifies \eqref{eq:SYM_smallLip}}.
\end{align}

Note also that if $|y| \geq \left< y, -e_x \right> \geq \delta_0$ (resp. $|y| \geq \left< y, -e_z \right> \geq \delta_0 |y|$), then 
\begin{align*}
& \left< K(y), \Omega(-e_x) \right>= - \left< K(y), \Omega(e_x) \right> \geq \frac{\delta_0}{2} \\
& \mbox{resp.  } - \left< K(y), \Omega(e_z) \right> \geq \frac{\delta_0}{2}.
\end{align*}

Thus, we may write
\begin{align}
    & \int\left( \left< K(-y), e_{\Omega(x)}\right> \left< y, e_x \right> + \left< K(-y), \nu \right> \left<y, e_z\right> \right) \frac{\vr'\ps{\av{\frac{y}{r}}^2}}{| y|^2} \, d\mu(y) \\
    & = \int_{\{|\left< y, e_x \right>| \geq \delta_0 |y| \, \mathrm{ and } \, |\left< y, e_z \right>| \geq \delta_0 |y|\}} \label{eq:SYM_int1}\\
    & + \int_{\{|\left< y, e_x\right>| \leq \delta_0 |y|\, \mathrm{but } \, |\left<y, e_z\right>| \geq \delta_0 |y| \}} \label{eq:SYM_int2}\\
    & + \int_{\{|\left< y, e_z\right>| \leq \delta_0 |y|\, \mathrm{but } \, |\left<y, e_x\right>| \geq \delta_0 |y| \}}. \label{eq:SYM_int3}
\end{align}
Indeed, notice that we cannot possibly have that both $|\left<y, e_x\right>| \leq \delta_0 |y|$ and $|\left<y, e_z\right>| \leq \delta_0 |y|$.
The integral in \eqref{eq:SYM_int1} can be immediately bounded below by
\begin{align}
    & \int_{\{|\left< y, e_x \right>| \geq \delta_0 |y| \, \mathrm{ and } \, |\left< y, e_z \right>| \geq \delta_0 |y|\}} \delta_0^2 |y|^2 \frac{\vr'\ps{\av{\frac{y}{r}}^2}}{|y|^2}\, d\mu(y) \\
    & \geq \frac{\delta_0^2}{r^2} \mu(\{|\left< y, e_x \right>| \geq \delta_0 |y| \, \mathrm{ and } \, |\left< y, e_z \right>| \geq \delta_0 |y|\} \cap A(0, r, 2r)).
\end{align}
As for the integral in \eqref{eq:SYM_int2}, we proceed as follows: by choosing $\delta_1>0$ appropriately, we can make sure that if 
\begin{align} \label{eq:SYM_111}
    |\left<y, e_x \right>| \leq \delta_0 |y|= \cos(\pi/2 - \delta_1)|y|,
\end{align}
then $|\left<K(y), \Omega(e_x)\right>| \leq 2 \delta_0 |y|$; thus for any $y$ satisfying \eqref{eq:SYM_111}, we have that
\begin{align}
    \left<y, e_x\right> \left<K(y), K(e_x)\right> \geq - 3\delta_0^2 |y|^2.
\end{align}
On the other hand, still for those $y$'s such that \eqref{eq:SYM_111}, it holds that
\begin{align}
    \cos(|\theta(y) - \theta(e_x)|)  \geq \sin\ps{\frac{\pi}{2}- \delta_1}. 
\end{align}
Hence we may write
\begin{align}
    & \int_{\{|\left< y, e_x\right>| \leq \delta_0 |y|\, \mathrm{but } \, |\left<y, e_z\right>| \geq \delta_0 |y| \}} \ps{ \left<y, e_x\right> \left<K(y), K(e_x)\right> + \left<y, e_z\right>\left<K(y), K(e_z)\right> } \frac{\vr'\ps{\av{\frac{y}{r}}^2}}{| y|^2} \, d\mu(y) \\
    & \gtrsim \int_{\{|\left< y, e_x\right>| \leq \delta_0 |y|\, \mathrm{but } \, |\left<y, e_z\right>| \geq \delta_0 |y| \}} |y|^2\ps{ - \cos^2\ps{\frac{\pi}{2}-\delta_1}  + \sin^2 \ps{\frac{\pi}{2} - \delta_1} } \frac{\vr'\ps{\av{\frac{y}{r}}^2}}{| y|^2} \, d\mu(y)\\
    & = \int_{\{|\left< y, e_x\right>| \leq \delta_0 |y|\, \mathrm{but } \, |\left<y, e_z\right>| \geq \delta_0 |y| \}} \ps{1 - 2 \cos^2\ps{\frac{\pi}{2} - \delta_1}} \, \vr'\ps{\av{\frac{y}{r}}^2} \, d\mu(y). \label{eq:SYM_121}
\end{align}
If we choose $\delta_1 \leq \frac{\pi}{6}$ (which determines $\delta_\Omega$), we obtain that 
$1 - 2 \sin(\delta_1) \geq \frac{1}{2}$, and therefore 
\begin{align}
    \eqref{eq:SYM_121} \geq \frac{1}{2} \mu \ps{\{|\left< y, e_x\right>| \leq \delta_0 |y|\, \mathrm{but } \, |\left<y, e_z\right>| \geq \delta_0 |y| \} \cap A(0, r, 2r)}.
\end{align}
We can estimate the integral in \eqref{eq:SYM_int3} in the same way; the three estimates together and the lower regularity of $\mu$ give the lemma.
\fi







\begin{align}
    \delta_\Omega \leq \frac{ \cos(\delta_1)}{\pi -\cos(\delta_1)}.
\end{align}
One can easily see that the function on the right hand side is bounded below by an absolute constant $\gamma \geq \frac{1}{10}$ if $\delta_1$ is small and positive.
\begin{remark}
In particular, this determines how small $\delta_\Omega$ has to be. 
\end{remark}
We have shown that, for $\delta_\Omega$ sufficiently small, if $\left< y, e_z \right> \geq \delta_0 |y|$ then also $\left<K(y), \Omega(e_z) \right> \gtrsim |y| \delta_0$. 
